A Simple and Flexible Modeling for Mental Disorder Detection by Learning from Clinical Questionnaires

Social media is one of the most highly sought resources for analyzing characteristics of the language by its users. In particular, many researchers utilized various linguistic features of mental health problems from social media. However, existing approaches to detecting mental disorders face critical challenges, such as the scarcity of high-quality data or the trade-off between addressing the complexity of models and presenting interpretable results grounded in expert domain knowledge. To address these challenges, we design a simple but flexible model that preserves domain-based interpretability. We propose a novel approach that captures the semantic meanings directly from the text and compares them to symptom-related descriptions. Experimental results demonstrate that our model outperforms relevant baselines on various mental disorder detection tasks. Our detailed analysis shows that the proposed model is effective at leveraging domain knowledge, transferable to other mental disorders, and providing interpretable detection results.

==> Img/criterion.tex <==
\label{subsec:case}
\begin{figure}[ht]
\centering
\includegraphics[width=0.8 \linewidth]{Img/probability.png}
\caption{Examples with symptoms of corresponding mental disorder. The \textit{label} indicates a gold standard, and the \textit{pred} indicates the prediction of our model.}
\label{fig:probability}
\vspace{-0.1in}
\end{figure}

==> Img/gpt-3_ex.tex <==
\begin{figure*}[ht]
\centering
\includegraphics[scale=0.7]{Img/gpt-3_ex.png}
\caption{The model architecture of Multi-Head Siamese network (MHS).
}
\label{fig:gpt3}
\vspace{-0.1in}
\end{figure*}
